A maximum likelihood estimate of natural mortality for brown tiger prawn (Penaeus esculentus) in Moreton Bay (Australia)

The delay difference model was implemented to fit 21 years of brown tiger prawn (Penaeus esculentus) catch in Moreton Bay by maximum likelihood to assess the status of this stock. Monte Carlo simulations testing of the stock assessment software coded in C++ showed that the model could estimate simultaneously natural mortality in addition to catchability, recruitment and initial biomasses. Applied to logbooks data collected from 1990 to 2010, this implementation of the delay difference provided for the first time an estimate of natural mortality for brown tiger prawn in Moreton Bay, equal to $0.031 \pm 0.002$ week$^{-1}$. This estimate is approximately 30\% lower than the value of natural mortality (0.045 week$^{-1}$) used in previous stock assessments of this species.

==> Tables/ModelComparison.tex <==
% latex table generated in R 3.0.2 by xtable 1.7-1 package
% Fri Nov 15 13:22:24 2013
%\begin{table}[ht]
\begin{sidewaystable}[ht]
\centering
\small
\begin{tabular}{lcccccccccc}
  \toprule
  Model & $p$ & AIC & \multicolumn{2}{c}{Catchability} & \multicolumn{2}{c}{Recruitment distribution} & \multicolumn{2}{c}{Initial biomasses} &  \multicolumn{1}{c}{} & \multicolumn{1}{c}{Natural mortality} \\  \cmidrule(r){1-1}
  \cmidrule(r){2-2}
  \cmidrule(r){3-3}
  \cmidrule(r){4-5}
  \cmidrule(r){6-7}
  \cmidrule(r){8-9}
  \cmidrule(r){10-10}
  \cmidrule(r){11-11}
   & & & $q_{1} \ (\times 10^{-4})$ & $q_{2} \ (\times 10^{-4})$ & $\mu$ & $\kappa$ & $B_{1} \ (\times 10^{5})$ & $B_{2} \ (\times 10^{5})$ & $\sigma$ & $M$\\
  \midrule
\input{Tables/ModelComparisonData.tex}
   \hline
\end{tabular}
\caption{Comparison between several models fitted to catch using a negative log-likelihood function. Results were ordered by increasing values of Akaike Information Criterion (AIC) from top to bottom.} 
\label{tab:ModelComparison}
\end{sidewaystable}
%\end{table}

